Finding Money Launderers Using Heterogeneous Graph Neural Networks

Current anti-money laundering (AML) systems, predominantly rule-based, exhibit notable shortcomings in efficiently and precisely detecting instances of money laundering. As a result, there has been a recent surge toward exploring alternative approaches, particularly those utilizing machine learning. Since criminals often collaborate in their money laundering endeavors, accounting for diverse types of customer relations and links becomes crucial. In line with this, the present paper introduces a graph neural network (GNN) approach to identify money laundering activities within a large heterogeneous network constructed from real-world bank transactions and business role data belonging to DNB, Norway's largest bank. Specifically, we extend the homogeneous GNN method known as the Message Passing Neural Network (MPNN) to operate effectively on a heterogeneous graph. As part of this procedure, we propose a novel method for aggregating messages across different edges of the graph. Our findings highlight the importance of using an appropriate GNN architecture when combining information in heterogeneous graphs. The performance results of our model demonstrate great potential in enhancing the quality of electronic surveillance systems employed by banks to detect instances of money laundering. To the best of our knowledge, this is the first published work applying GNN on a large real-world heterogeneous network for anti-money laundering purposes.

==> old4_data.tex <==
\section{AML use case}
\label{data}

This section describes the heterogeneous graph which are subjects of the experiments in this paper.
The graph is established based on custom and transaction data from Norway's largest bank, DNB, in the period ... to ....
%The main ingredient in the graph is all transactions to or from customers in Norway's largest bank from in the period ... to .... Additionally, the graph includes basic data about the customers, and professional role relationships individuals may have in companies in the graph.
The nodes in the graph represent entities that are senders and recipients of the financial transactions.
If two entities participate in a transaction with each other, this is represented by an edge between the two, where the direction of the edge points from the sender to the recipient.
There are in total 5 million nodes and 9 million such edges in the graph. 

There are three types of nodes in the graph. 
The first one is called individual, and represents a human individual’s customer relationship in the bank. 
It includes all of the individual’s accounts in the bank\footnote{ 
Transactions made to or from any of the accounts in the bank belonging to the customer will result in an edge to or from the node representing the individual. 
}.
The second type of node is called organisation, and represents an organisation’s or company’s customer relationship in the bank in the same manner as for a node representing an individual. 
The third type of node is called external, and represents a sender or recipient in a transaction which is outside of the bank. 
%
The majority of the edges in the graph represent presence of a financial transactions between different individuals/organizations/external entities in the edge direction. 
In addition to this edge type, the graph includes a second edge type: role.
This edge points from an individual to an organisation if the individual occupy a position in the board, is the CEO, or holds an ownership in the organisation. 
%
The resulting graph is directed and heterogeneous with respect to both nodes and edges. 
Figure \ref{fig:graph_schema} shows the schema of the graph, including the nine possible meta-steps. 


\begin{figure}[!t]
\centering
\includegraphics[width=0.6\linewidth]{figures/graph_schema.pdf}
\caption{The schema of the graph that has been the subject of our experiments, with the nodes representing customer relationships in DNB outlined by the grey ellipse. Here, the transaction-edges are abbreviated as \textit{Txn}. }
\label{fig:graph_schema}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Due to the sensitive nature of these data, we cannot reveal the exact definitions of the features assoicated with the different nodes/edges in our model, but the in the following we give a broad overview.

The three node types have separate set of features which contain basic information about the entity such as age, gender and nationality.
The transaction edges contains aggregated transactions between the sender and recipient during a one year period, and has as features the number and monetary amount of transactions made. I.e.~multiple transactions between to entities are only represented by a single edge (per direction), while the number of transactions and their 
The role edges, on the other hand, have no features. 

The nodes that represent customers of the bank, i.e.~individuals and organisations, are assigned a
binary class (0 for regular customers, 1 for suspicious customers). 
Suspicious customers are defined as customers that have been subject of an AML case (stage 2\footnote{
Note that customers implicated in cases that were not reported to the FIU, are still defined as suspicious.  
This decision was made because our objective is to model suspicious activity, which these customers certainly have conducted, even though the suspiciousness was diminished by a close manual inspection.
} 
in Figure \ref{fig:alert_workflow}) during a certain (non-disclosable) time window. Approximately 0.8\% of the customer nodes belong to class 1.  

In addition to the original node features, we include four types of network features: Degree summary, centrality metrics, DeepWalk embeddings and Metapath2Vec embeddings. 
Combined, they are an attempt to incorporate high-quality features on the node-level that summarize information about their role in the heterogeneous network. 
In total, this results in 79 additional features. 
Combined with the entity features we end up with 87 and 86 features for individuals and organisations, respectively. Precise specification of these network features are provided in \ref{app:network_features}.



==> old5_experiment.tex <==

%\clearpage
\section{AML use case}
\label{Experiment}

%In this section, we compare the performance of our HMPNN model to a rich set of existing GNNs using the AML-graph described in Section \ref{data}. 
In this section we test our HMPNN model on the AML scenario and data described in Section \ref{data}. In particular, we are interested in the ability of the method to predict the label (suspicious or not) on nodes where the label is unknown to the model.
To better understand how well suited our HMPNN model is for this use case, we compare its performance to a rich set of existing GNNs.

We start by describing the technical modeling regime and the benchmark methods. We then present the training/testing regime and the evaluation measures, before the results are presented and discussed.

\subsection{Technical Circumstances}
Our HMPNN model is implemented in Python, using the library PyTorch Geometric (PyG) \citep{Fey2019FastGR}. 
PyG is an open source python library built upon \textit{PyTorch}
\footnote{PyTorch is an open source deep learning library used for applications such as image analysis and natural language processing. It achieves high computational performance of tensor computing by utilizing graphics processing units (GPUs) through \textit{Compute Unified Device Architecture} (CUDA).}
\citep{NEURIPS2019_9015}, which specialises in  utilities for representing and training GNNs. 
PyG is the most popular library for working with GNNs, and most of the methods we benchmark against (see Section \ref{sec:benchmark_methods}) are also implemented in PyG, making it a convenient comparison framework for our experiment.

All modelling in this section were carried out in \textit{python 3.7.0}. 
The computer had 8 CPUs of the type \textit{High frequency Intel Xeon E5-2686 v4 (Broadwell) processors}, with 61GB shared memory, and one GPU of type \textit{NVIDIA Tesla V100} with 16GB memory. The GPU has 5,120 CUDA Cores and 640 Tensor Cores.


\subsection{Benchmark methods}
\label{sec:benchmark_methods}

We compare our HMPNN model against the following five methods: Basic 2-layer neural network with graph features,
Heterogeneous GraphSage,
HAN,
MAGNN, and % - Not done in thesis but would be interesting....
GINEConv. % It is homogeneous, but can utilize edge features. https://arxiv.org/abs/1905.12265 
% "Explicit Message-Passing Heterogeneous Graph Neural Network" Benchmarks against GCN, GAT, GIN, RGCN, HAN. I'm not sure how they apply the first four models to a heterogeneous graph, given that they don't allow message passing between nodes with different dimension of feature vectors. One approach could be to first map all feature vectors to a vector of the same length, and proceed in the same manner as done with graphsage in the thesis. 

The specifics of these methods are described below. 

\subsubsection{2-layer neural network with graph features}

To get a feeling of the performance improvement due to the use of methods utilizing the graph structure of the data, we include a non-GNN baseline method in our comparison. 
We used a purely entity-based two-layer neural network classifier, where the graph is only used upstream to create additional network features for each node which is added to its intrinsic entity level features. 

We created four types of network features: Degree summary, centrality metrics, DeepWalk embeddings
and Metapath2Vec embeddings. Combined, they are an attempt to incorporate high-quality features
on the node-level that summarize information about their role in the heterogeneous network. In
total, this results in 79 additional features. Combined with the entity features
we end up with 87 and 86 features for individuals and organisations, respectively. Precise specification of these network features are provided in \ref{app:network_features}.
This model was trained with PyTorch.

\subsubsection{GraphSage}
The second benchmark model is GraphSage. 
Because this message operator does not utilize the edge features, it does not initially have any information about the quantity of money that flows between the nodes. 
Therefore, there is reason to believe that the model will benefit from adding the additional degree features.

\subsubsection{HAN}
The (second/third ??) benchmark model is HAN. 
We used the implementation of HAN in PyG. 

Here, we set the hidden representation vector dimension to 8 for each embedding and for each node type in the hidden layers. We set the number of heads to 1. 
The resulting messages from neighboring nodes go through an additional SLP in each layer (with separate parameters for each node type) which outputs the new embeddings.

\subsubsection{MAGNN}


\subsubsection{GINEConv}



\subsection{Experiment setup}
The goal of this use case and benchmark is to compare the different methods ability to predict the label on nodes where the label is unknown to the model. To mimic such a scenario, we split the nodes into a training set and a test set. The whole graph is available for each of the models, but the labels are only available for the nodes in the training set. Then at testing time, the each method attempts to predict the (unknown) nodes in the test set, and their performance is compare using different performance measures.
In this experiment, we applied a 70-30 train-test split, where the splitting was performed using stratified random sampling with allocation proportional to the original class balance, such that the class balance is preserved in the two sets. The same split was used for all methods.

All models where trained with the Adam optimiser \citep{Kingma2015Adam}, using the Binary Cross Entropy
\[
\text{Loss}(\hat{y}_v, y_v) = y_v\cdot \log(\hat{y}_v) + (1-y_v)\cdot \log(1-\hat{y}_v).
\]
%

The hyperparameters were tuned using 5-fold cross-validation on the training set. Here, three hyperparameters were determined: (1) The regularization strength. (2) The learning rate. (3) The Number of training-iterations, i.e. by early stopping. 
For all experiments carried out, the learning rate was in the range $[10^{-4},10^{-1}]$. As for regularization, the $L_2$-constraint was used, and was in the range $[10^{-8},10^{-1}]$. The optimal value for the $L_2$-constraint was highly dependent on the complexity of the model to be trained.  


\subsection{Performance measures}

\subsection{Results}

\clearpage

\begin{table}[t]
    \centering
    \small
    \caption{Results logistic regression and neural network with 1 and 2 hidden layers. Here, 1 is logistic regression, and 2/3 are neural network with 1/2 hidden layers, respectively. Totally 98 node features, where 11 are intrinsic, 15 are summary of node-neighborhoods (counts number of different meta-steps), 8 are weighted summary of edges where the weight is the transaction-sums, and 64 are metapath2vec embeddings (8x8, dimension 8 for each of the 8 meta-steps an individual node is part of.)}
    \label{tab:...}
\begin{tabular}{ccccccccc}
\hline
\multicolumn{1}{c}{Number}   & Degree   && \multicolumn{4}{c}{Recall(\%)}  &  \multicolumn{1}{c}{PR} & \multicolumn{1}{c}{ROC} \\ \cline{4-7}
\multicolumn{1}{c}{of Layers}  & Features&& 1  & 5  & 10 & 50 & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{AUC} \\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{1}}  &\multicolumn{1}{c}{\multirow{2}{*}{No}}    & Precision(\%)     & 61.54 & 36.28 & 28.55 & 5.53   &  \multirow{2}{*}{ 0.1075 } &  \multirow{2}{*}{ 0.8547 } \\
                                                                &                                           &Lift               & 135.96 & 80.16 & 63.07 & 12.23  &                           &\\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{2}}  &\multicolumn{1}{c}{\multirow{2}{*}{No}}    & Precision(\%)     & 64.00 & 43.82 & 30.51 & 5.89   &  \multirow{2}{*}{ 0.1173 } &  \multirow{2}{*}{ 0.8613 } \\
                                                                &                                           &Lift               & 141.40 & 96.82 & 67.41 & 13.01  &                           &\\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{3}}  &\multicolumn{1}{c}{\multirow{2}{*}{No}}    & Precision(\%)     & 61.54 & 47.56 & 34.68 &5.88   &  \multirow{2}{*}{ 0.1237} &  \multirow{2}{*}{ 0.8612 } \\
                                                                &                                           &Lift               & 135.96 & 105.08 & 76.61 & 13.00  &                           &\\ 
\hline
\end{tabular}
\end{table}


\begin{table}[t]
    \centering
    \small
    \caption{Results from graphSage-models }
    \label{tab:...}
\begin{tabular}{ccccccccc}
\hline
\multicolumn{1}{c}{Number}   & Degree   && \multicolumn{4}{c}{Recall(\%)}  &  \multicolumn{1}{c}{PR} & \multicolumn{1}{c}{ROC} \\ \cline{4-7}
\multicolumn{1}{c}{of Layers}  & Features&& 1  & 5  & 10 & 50 & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{AUC} \\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{1}}  &\multicolumn{1}{c}{\multirow{2}{*}{No}}    & Precision(\%)     & 59.26 & 33.62 & 20.58 & 4.01   &  \multirow{2}{*}{ 0.0836 } &  \multirow{2}{*}{ 0.8329 } \\
                                                                &                                           &Lift               & 130.93 & 74.28 & 45.48 & 8.86  &                           &\\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{2}}  &\multicolumn{1}{c}{\multirow{2}{*}{No}}    & Precision(\%)     & 61.54 & 48.15 & 38.56 & 6.51   &  \multirow{2}{*}{ 0.1280 } &  \multirow{2}{*}{ 0.8879 } \\
                                                                &                                           &Lift               & 135.96 & 106.38 & 85.19 & 14.39  &                           &\\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{3}}  &\multicolumn{1}{c}{\multirow{2}{*}{No}}    & Precision(\%)     & 59.26 & 60.47 & 42.47 &7.19   &  \multirow{2}{*}{ 0.1452} &  \multirow{2}{*}{ 0.8960 } \\
                                                                &                                           &Lift               & 130.93 & 133.59 & 93.82 & 15.88  &                           &\\ 
\hline
\end{tabular}
\end{table}



\begin{table}[t]
    \centering
    \small
    \caption{Results from graphSage-models with additional node-features. The nodes representing Individual, LegalPerson and UnknownEntity have gotten 8, 8 and 6 extra node features, respectively. The features are the weighted in/out degrees for the transaction-edges, and the weight is the transaction-amount on the edges.}
    \label{tab:...}
\begin{tabular}{ccccccccc}
\hline
\multicolumn{1}{c}{Number}   & Degree   && \multicolumn{4}{c}{Recall(\%)}  &  \multicolumn{1}{c}{PR} & \multicolumn{1}{c}{ROC} \\ \cline{4-7}
\multicolumn{1}{c}{of Layers}  & Features&& 1  & 5  & 10 & 50 & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{AUC} \\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{1}}  &\multicolumn{1}{c}{\multirow{2}{*}{Yes}}    & Precision(\%)     & 48.48 & 34.21 & 21.29 & 4.24   &  \multirow{2}{*}{ 0.0858 } &  \multirow{2}{*}{ 0.8405 } \\
                                                                &                                           &Lift               & 107.12 & 75.59 & 47.04 & 9.36  &                           &\\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{2}}  &\multicolumn{1}{c}{\multirow{2}{*}{Yes}}    & Precision(\%)     & 64.00 & 50.65 & 35.39 & 7.41   &  \multirow{2}{*}{ 0.1368 } &  \multirow{2}{*}{ 0.8882 } \\
                                                                &                                           &Lift               & 141.40 & 111.91 & 78.19 & 16.38  &                           &\\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{3}}  &\multicolumn{1}{c}{\multirow{2}{*}{Yes}}    & Precision(\%)     & 69.57 & 50.32 & 38.27 &7.68   &  \multirow{2}{*}{ 0.1424} &  \multirow{2}{*}{ 0.8915 } \\
                                                                &                                           &Lift               & 153.70 & 111.18 & 84.56 & 16.98  &                           &\\ 
\hline
\end{tabular}
\end{table}



\begin{table}[t]
    \centering
    \small
    \caption{Results from mpnn-models }
    \label{tab:...}
\begin{tabular}{ccccccccc}
\hline
\multicolumn{1}{c}{Number}   & Degree   && \multicolumn{4}{c}{Recall(\%)}  &  \multicolumn{1}{c}{PR} & \multicolumn{1}{c}{ROC} \\ \cline{4-7}
\multicolumn{1}{c}{of Layers}  & Features&& 1  & 5  & 10 & 50 & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{AUC} \\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{1}}  &\multicolumn{1}{c}{\multirow{2}{*}{No}}    & Precision(\%)     & 64.00 & 38.24 & 29.75 & 5.34   &  \multirow{2}{*}{ 0.1090 } &  \multirow{2}{*}{ 0.8401 } \\
                                                                &                                           &Lift               & 141.40 & 84.48 & 65.73 & 11.80  &                           &\\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{2}}  &\multicolumn{1}{c}{\multirow{2}{*}{No}}    & Precision(\%)     & 69.57 & 42.62 & 36.38 & 7.76   &  \multirow{2}{*}{ 0.1359 } &  \multirow{2}{*}{ 0.8863 } \\
                                                                &                                           &Lift               & 153.70 & 94.17 & 80.39 & 17.14  &                           &\\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{3}}  &\multicolumn{1}{c}{\multirow{2}{*}{No}}    & Precision(\%)     & 84.21 & 53.79 & 38.27 &8.67   &  \multirow{2}{*}{ 0.1532} &  \multirow{2}{*}{ 0.8955 } \\
                                                                &                                           &Lift               & 186.06 & 118.85 & 84.56 & 19.16  &                           &\\ 
\hline
\end{tabular}
\end{table}

\begin{table}[t]
    \centering
    \small
    \caption{Results from hmct-models }
    \label{tab:...}
\begin{tabular}{ccccccccc}
\hline
\multicolumn{1}{c}{Number}   & Degree   && \multicolumn{4}{c}{Recall(\%)}  &  \multicolumn{1}{c}{PR} & \multicolumn{1}{c}{ROC} \\ \cline{4-7}
\multicolumn{1}{c}{of Layers}  & Features&& 1  & 5  & 10 & 50 & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{AUC} \\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{1}}  &\multicolumn{1}{c}{\multirow{2}{*}{No}}    & Precision(\%)     & 76.19 & 48.75 & 38.18 & 6.92   &  \multirow{2}{*}{ 0.1418 } &  \multirow{2}{*}{ 0.8801 } \\
                                                                &                                           &Lift               & 168.34 & 107.71 & 84.35 & 15.28  &                           &\\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{2}}  &\multicolumn{1}{c}{\multirow{2}{*}{No}}    & Precision(\%)     & 61.54 & 50.65 & 43.66 & 8.96   &  \multirow{2}{*}{ 0.1555 } &  \multirow{2}{*}{ 0.8989 } \\
                                                                &                                           &Lift               & 135.96 & 111.91 & 96.47 & 19.80  &                           &\\ 
\hline
\multicolumn{1}{c}{\multirow{2}{*}{3}}  &\multicolumn{1}{c}{\multirow{2}{*}{No}}    & Precision(\%)     & 66.67 & 58.21 & 50.99 &10.25   &  \multirow{2}{*}{ 0.1800} &  \multirow{2}{*}{ 0.9083 } \\
                                                                &                                           &Lift               & 147.29 & 128.61 & 112.65 & 22.65  &                           &\\ 
\hline
\end{tabular}
\end{table}


\clearpage
Number of model parameters for modelLogisticRegression: 99\\
Number of model parameters for modelNeuralNetwork\_1: 9,801\\
Number of model parameters for modelNeuralNetwork\_2: 19,503\\

Number of model parameters for modelSageConv1Layer: 189\\
Number of model parameters for modelSageConv2Layer: 3,999\\
Number of model parameters for modelSageConv3Layer: 7,809\\
Number of model parameters for modelNNConv1Layer: 296\\
Number of model parameters for modelNNConv2Layer: 6,536\\
Number of model parameters for modelNNConv3Layer: 12,776\\
Number of model parameters for modelHmct1Layer: 3,071\\
Number of model parameters for modelHmct2Layer: 4,487\\
Number of model parameters for modelHmct3Layer: 6,303\\

Number of model parameters for modelSageConv1Layer with additional node-features: 329\\
Number of model parameters for modelSageConv2Layer with additional node-features: 13,045\\
Number of model parameters for modelSageConv3Layer with additional node-features: 25,761\\
Number of model parameters for modelSageConv3Layer with additional node-features: 25,761\\
Number of model parameters for modelSageConv3Layer with additional node-features: 25,761\\

==> old8_notes.tex <==
\begin{comment}
\subsection{Heterogeneous MPNN - OLD}
NOTES: \\
Expressing this using $v^{\nu}$ doesn't work, because one can't have a symbol with super/sub-script in a super/sub-script: \text{A\_A\_A} does not work!!!!!
\\
I don't think $s$ works... 
\\

Our heterogeneous formulation of the MPNN method can now be expressed.

The representation of all nodes are initialized as their feature vector:
\[
\b{h}_v^{(0)} = \b{x}_v^{\nu}, \; \forall \; \b{x}_v^{\nu} \in \b{X}^{\nu}, \nu \in Q^V.
\]

In each iteration $k = 1,\dots, K$, MPNN message passing will be performed for each meta-step that exists in the graph $s = (\mu, \varepsilon, \nu) \in S$.

For each meta-step $s = (\mu, \varepsilon, \nu) \in S$, we perform MPNN message passing for all nodes of type $\nu$:

\begin{align*}
    \b{m}_v^{(s,k)} &= \sum_{u\in N_s(v)} M_k^s(\b{h}_v^{(k-1)}, \b{h}_u^{(k-1)}, \b{r}_{uv}^{\varepsilon}),\; \forall v \in V^{\nu} \\
    \b{h}_v^{(s,k)} &= U_k^s( \b{h}_v^{(k-1)}, \b{m}_v^{(s,k)})
\end{align*}

For each node $v$, aggregate the representations over the meta-steps $s \in S$:
\[
    \b{h}_v^{(k)} = \underset{s \in S}{\text{AGG}} ( \b{h}_v^{(s,k)} )
\]
\end{comment}

\begin{comment}
\subsubsection{MPNN}
\textbf{From \cite{WU2020}, but modified}: 

Message Passing Neural Network (MPNN) \citep{GILMER2017} outlines a general framework of spatial-based ConvGNNs. 
It treats graph convolutions as a message passing process in which information can be passed from one node to another along edges directly. MPNN runs $k$-step message passing iterations to let information propagate further. 
The message passing function is defined as
\begin{align*}
    \b{m}_v^{(k)} &= \sum_{u\in N(v)} M_k(\b{h}_v^{(k-1)}, \b{h}_u^{(k-1)}, \b{r}_{uv}), \\
    \b{h}_v^{(k)} &= U_k( \b{h}_v^{(k-1)}, \b{m}_v^{(k)})
\end{align*}
where $\b{h}_v^{0} = \b{x}_v$, $U_k(\cdot)$ and $M_k(\cdot)$ are functions with learnable parameters, and are called the \textit{node updated functions} and the \textit{message functions}, respectively.
After deriving the hidden representations of each node, $\b{h}_v^{(K)}$ can be passed to an output layer to perform node-level prediction tasks.
MPNN cover many existing GNNs by assuming different forms of $U_k(\cdot)$ and $M_k(\cdot)$, such as \cite{KIPF2016}.
\end{comment}

\begin{comment}
\begin{definition}(Adjacency matrix)
The adjacency matrix $\boldsymbol{A}$ of a graph $G = (V, E)$ is an $n\times n$ matrix with $\boldsymbol{A}_{ij}=1$ if $e_{ij}\in E$ and $\boldsymbol{A}_{ij} = 0$ if $e_{ij} \neq E$. 
\end{definition}

\begin{definition}(Node neighborhood (homogeneous))
\label{def:neighborhood}
The neighborhood of a node $v$ is defined as $N(v) = \{u \in V|(v,u) \in E\}$. 
\end{definition}
\end{comment}

\begin{comment}
\begin{definition}(Heterogeneous graph - OLD)
\label{def:heteroGraph}
A heterogeneous graph is represented as $G = (V, E, \boldsymbol{X}, \boldsymbol{R}, \phi, \psi)$ where $V$ is the set of nodes, and $E$ is the set of edges. 
Let $v\in V$ denote a node and $e_{uv}=(u,v)\in E$ an edge pointing from $v$ to $u$. 
Let $\phi : V \rightarrow Q^V$ represent a node type mapping function and $\psi : E \rightarrow Q^E$ an edge type mapping function.
Here, $Q^V$ and $Q^E$ denote finite sets of predefined node types and edge types, respectively.
Each node $v$ of type $\nu = \phi(v)$ is also associated with features $\boldsymbol{X}_v^{\nu}$, while each edge $e_{uv}$ of type $\varepsilon = \psi(e_{uv})$ with feature $\boldsymbol{R}_{uv}^{\varepsilon}$.\\
Note: This needs to change: $\psi(e_{uv})$ returns a subset of edge types in $Q^E$, which are are edge types that point from node $u$ to node $v$.
\end{definition}
\end{comment}

\begin{comment}
Another example with particular relevance for this paper is graphSage \citep{HAMILTON2017}. This paper considers a few different approaches, but one of them can be expressed as follows:
\begin{align*}
    M_k(\b{h}_v^{(k-1)}, \b{h}_u^{(k-1)}, \b{r}_{uv}) &= \b{W}_k \b{h}_u^{(k-1)}, \\
    U_k\big(\b{h}_v^{(k-1)}, \b{m}_v^{(k)}\big) &= \sigma\big(\b{m}_v^{(k)} + \b{B}_k \b{h}_v^{(k-1)} \big).
\end{align*}
 Here, $\sigma(\cdot)$ is the sigmoid function. 
\end{comment}


\begin{comment}
\subsection{Heterogeneous MPNN - OLD}

For a specific meta-step $s = (\mu, \varepsilon, \nu)$, all nodes $v\in V$ with type $\phi(v) = \nu$ will receive messages from the neighborhood that corresponds to the meta-step: $N_{\mu}^{\varepsilon}(v)$.
%
Each meta-step will have their own message function and node update function with parameters that will be learned for that specific meta-step.
We denote these functions $M_k^s(\cdot)$ and $U_k^s(\cdot)$ for iteration $k$ and meta-step $s$.
%
The message passing equation \eqref{eq_mpnn} can be expressed for a specific meta-step as follows:
\begin{align*}
    \b{m}_v^{(s,k)} &= \sum_{u\in N_{\mu}^{\varepsilon}(v)} M_k^s(\b{h}_v^{(k-1)}, \b{h}_u^{(k-1)}, \b{r}_{uv}^{\varepsilon}),\;\forall\; v\in V, s = (\mu, \varepsilon, \phi(v)) \in S, \\
    \b{h}_v^{(s,k)} &= U_k^s( \b{h}_v^{(k-1)}, \b{m}_v^{(s,k)}).
\end{align*}

After the above equations have been performed for each meta-step at a certain iteration, a node $v$ will have multiple meta-step-specific representations $\b{h}_v^{(s,k)}$. These will be aggregated to produce the new representation vector $\b{h}_v^{(k)}$:
\[
    \b{h}_v^{(k)} = A\big( 
    \{
    \b{h}_v^{(s,k)} | s = (\mu, \varepsilon, \phi(v)) \in S
    \}  
    \big)
\]
\end{comment}


\begin{comment}
Our study has two contributions:
\begin{enumerate}
    \item Exploring the potential of applying supervised learning methods on a heterogeneous transaction-network to detect money laundering activities. 
    The dataset is realistic and created from real-world data, which makes the results representative to the real application. 
    \item Exploring various graph neural network architectures on a large real-world heterogeneous network, where the task is node classification. We expand upon methods and architectures in the literature, and construct a model especially suitable for the presented data. 
\end{enumerate}
\end{comment}


\begin{comment}
\clearpage
\begin{algorithm}
\caption{Heterogeneous MPNN }\label{alg:HMPNN}
\begin{algorithmic}
\State Initialize the representation of each node as its feature vector,
\[
\b{h}_v^{(0)} = \b{x}_v^{\nu}, \;\forall\; \b{x}_v^{\nu} \in \b{X}^{\nu}, \nu \in Q^V.
\]

\For{$k = 1,\dots, K$} \Comment{For each iteration}
\For{$\nu \in Q^V$} \Comment{For each node type in the graph}
\For{$v \in V,\; \phi(v) = \nu $} \Comment{For each node with node type $\nu$}
\For{$s = (\mu, \varepsilon, \nu)\in S$} \Comment{For each meta-step ending at $\nu$}

\State Compute the new representation for node $v$ for the specific
\State meta-step,
\[
\begin{aligned}
    \b{m}_v^{(s,k)} &= \sum_{u\in N_{\mu}^{\varepsilon}(v)} M_k^s(\b{h}_v^{(k-1)}, \b{h}_u^{(k-1)}, \b{r}_{uv}^{\varepsilon}), \\
    \b{h}_v^{(s,k)} &= U_k^s( \b{h}_v^{(k-1)}, \b{m}_v^{(s,k)}).
\end{aligned}
\]
\EndFor
\State Aggregate the representations from the multiple meta-steps into a 
\State single new representation for that node,
\State
\[
    \b{h}_v^{(k)} = A_k^{\nu}\big( 
    \{
    \b{h}_v^{(s,k)} \mid s = (\mu, \varepsilon, \phi(v)) \in S
    \}  
    \big)
\]
\EndFor
\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}
\clearpage
\end{comment}



\begin{comment}
\clearpage
\begin{algorithm}
\caption{Heterogeneous MPNN II }\label{alg:HMPNN}
\footnotesize
\begin{algorithmic}
\State Initialize the representation of each node as its feature vector,
\[
\b{h}_v^{(0)} = \b{x}_v^{\nu}, \;\forall\; \b{x}_v^{\nu} \in \b{X}^{\nu}, \nu \in Q^V.
\]

\For{$k = 1,\dots, K$} \Comment{For each iteration}
\For{$\nu \in Q^V$} \Comment{For each node type in the graph}
\For{$v \in V$, such that $\phi(v) = \nu $} \Comment{For each node with node type $\nu$}
\For{$\mu \in Q^V, \varepsilon \in Q^E$ such that $N_{\mu}^{\varepsilon}(v) \neq \emptyset$} \Comment{For each meta-step ending at $\nu$}

\State Compute the new representation for node $v$ for the specific
\State meta-step,
\[
\begin{aligned}
    \b{m}_v^{(\mu, \varepsilon,k)} &= \sum_{u\in N_{\mu}^{\varepsilon}(v)} M_k^{\mu, \varepsilon}(\b{h}_v^{(k-1)}, \b{h}_u^{(k-1)}, \b{r}_{uv}^{\varepsilon}), \\
    \b{h}_v^{(\mu, \varepsilon,k)} &= U_k^{\mu, \varepsilon}( \b{h}_v^{(k-1)}, \b{m}_v^{(\mu, \varepsilon,k)}).
\end{aligned}
\]
\EndFor
\State Aggregate the representations from the multiple meta-steps into a 
\State single new representation for that node,
\State
\[
    \b{h}_v^{(k)} = A_k^{\nu}\big( 
    \{
    \b{h}_v^{(\mu, \varepsilon,k)} \mid \mu \in Q^V, \varepsilon \in Q^E
    \}  
    \big)
\]
\EndFor
\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}
\end{comment}

\begin{comment}
\clearpage
\begin{algorithm}
\caption{Heterogeneous MPNN II MJ}\label{alg:HMPNN}
\footnotesize
\begin{algorithmic}
\State Initialize the representation of each node as its feature vector,
\[
\b{h}_v^{(0)} = \b{x}_v^{\nu}, \;\forall\; \b{x}_v^{\nu} \in \b{X}^{\nu}, \nu \in Q^V.
\]

\For{$k = 1,\dots, K$} \Comment{For each iteration}
\For{$v \in V$} \Comment{For each node}
\For{$\mu \in Q^V, \varepsilon \in Q^E$ such that $N_{\mu}^{\varepsilon}(v) \neq \emptyset$} \Comment{For each meta-step ending at $\phi(v)$}

\State Compute the new representation for node $v$ for the specific
\State meta-step,
\[
\begin{aligned}
    \b{m}_v^{(\mu, \varepsilon,k)} &= \sum_{u\in N_{\mu}^{\varepsilon}(v)} M_k^{\mu, \varepsilon}(\b{h}_v^{(k-1)}, \b{h}_u^{(k-1)}, \b{r}_{uv}^{\varepsilon}), \\
    \b{h}_v^{(\mu, \varepsilon,k)} &= U_k^{\mu, \varepsilon}( \b{h}_v^{(k-1)}, \b{m}_v^{(\mu, \varepsilon,k)}).
\end{aligned}
\]
\EndFor
\State Aggregate the representations from the multiple meta-steps into a 
\State single new representation for that node,
\State using the aggregation function, $A_k^{\nu}$ of node type $\nu=\phi(v)$
\State
\[
    \b{h}_v^{(k)} = A_k^{\nu}\big( 
    \{
    \b{h}_v^{(\mu, \varepsilon,k)} \mid \mu \in Q^V, \varepsilon \in Q^E
    \}  
    \big)
\]
\EndFor

\EndFor
\end{algorithmic}
\end{algorithm}
\clearpage
\end{comment}





\begin{comment}
\clearpage
Using this framework, multiple different GNNs can be defined by different choices of  $U_k(\cdot)$ and $M_k(\cdot)$.
For example, GCN \citep{KIPF2016} can be expressed as 
\begin{align*}
M_k(\b{h}_v^{(k-1)}, \b{h}_u^{(k-1)}, \b{r}_{uv}) &=\frac{\b{r}_{uv}}{\sqrt{\hat{d}_u\hat{d}_v}}\b{h}_u^{(k-1)},\\   
U_k(\b{h}_v^{(k)}, \b{m}_v^{(k+1)}) &=\text{ReLU}(W_k \b{m}_v^{(k+1)}),
\end{align*}
where $\hat{d}_v = 1 + \sum_{u\in V}\b{r}_{uv}$. Note that $\b{r}_{uv}$ is here restricted to being a scalar rather than a vector, resulting from that GCN is defined on (possibly) weighted graphs, but not on graphs with multiple edge features\footnote{From \citep{KIPF2016}: "Our framework currently does not naturally support edge features and is limited to undirected graphs (weighted or unweighted)."}.

\cite{GILMER2017} use 
$U_t = \text{GRU}(h_v^t, m_v^{t+1})$
as node update function, where $\text{GRU()}$ is the gated recurrent unit from \cite{CHO2014}. $\text{GRU()}$ is also used in \textit{Gated Graph Neural Networks} \citep{LI2016}.
%
As for the message function, they experiment with a few alternatives, one of which being 
\[
    M_k(\b{h}_v^{(k-1)}, \b{h}_u^{(k-1)}, \b{r}_{uv}) = g_k(\b{r}_{uv}) \b{h}_u^{(k-1)}.
\]
Here, $g_k(\cdot)$ is a neural network which maps $\b{r}_{uv}$ to a $d\times d$ matrix, where $d$ is the dimension of the representation vectors. 
From the viewpoint of the present work, this message passing function is essential, because it defines a learned message function that utilize edge features. 
Many other proposed GNNs such as GCN \citep{KIPF2016}, graphSage \citep{HAMILTON2017}, GAT \citep{VELIVCKOVIC2017}, RGCN \citep{SCHLICHTKRULL2018} and HAN \citep{WANG2019} do not incorporate edge features, and they therefore falls short on our graph. 
\clearpage
\end{comment}


\begin{comment}
However, these definitions do not allow multiple edges with the same direction between the same two nodes. We require a definition that incorporates a directed graph with multiple node types and multiple edge types, which also can have multiple edges between the same two nodes as long as the edges have different types. In addition, both nodes and edges have features which depends on their types. Here is our definition:
\end{comment}







==> old9_notations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\section{Notations}
Notation rules
\begin{enumerate}
    \item Bold uppercase characters to denote matrices.
    \item Bold lowercase characters denote vectors.
    \item Uppercase characters to denote sets. 
    \item Don't use mathcal/mathbb etc. 
    \item Subscript: ??
    \item Superscript: ??
\end{enumerate}



\begin{table}[!ht]\label{tbl:notation}
    \centering
    \footnotesize
    \caption{Notations}
    \begin{tabular}{ll}
        \hline
        Notation & Description \\
        \hline
        $n$ & The number of nodes. \\
        $m$ & The number of edges.\\
        $d$  & The dimension of a node feature vector. \\
        $c$ & The dimension of an edge feature vector. \\
        \hline
        $G$ & A (heterogeneous) graph. \\
        $\boldsymbol{A}$ & The adjacency matrix of a graph. \\
        \hline
        $V$ & The set of nodes in a graph. \\
        $u, v$ & A node $u,v\in V$.\\
        $\boldsymbol{X}\in \mathbb{R}^{n\times d}$ & The node feature matrix of a graph.\\
        $E$ & The set of edges in a graph. \\
        $e \in E$ & An edge in the graph. \\
        $e_{ij} \in E$ & An edge from node $v_i$ to $v_j$. \\
        $e_{uv} \in E$ & An edge from node $u$ to node $v$. \\
        $\boldsymbol{R}\in \mathbb{R}^{m\times c}$ & The edge feature matrix of a graph.\\
        $N(v) = \{v \in V|(v,u) \in E\}$ & The neighbors of a node $v$. \\ 
        \hline
        $\boldsymbol{W}, \boldsymbol{\Theta}, w, \theta$ & Learnable model parameters. \\
        \hline
        $M(\cdot)$& Message function. \\
        $U(\cdot)$& Node update function. \\
        $A(\cdot)$& Aggregation function. \\
        $\b{h}_v$& Representation of node $v$.\\
        $\b{m}_v$& Aggregated messages received by node $v$ from its neighborhood.\\
        $k$ & Iteration index. \\
        \hline
        $Q^V$ & The set of node types in a graph.\\
        $Q^E$ & The set of edge types in a graph.\\
        $\phi(v)$ & The node type mapping function $\phi : V \rightarrow Q^V$. \\
        $\psi(e)$ & The edge type mapping function $\psi : E \rightarrow Q^E$. \\
         $\nu, \mu \in Q^V$ & A specific node type. \\
         $\varepsilon \in Q^E$ & A specific  edge type. \\
        $S$ & The set of meta steps in the graph. \\
        $s = \{(\mu,\varepsilon,\nu) \in S\}$ & A specific meta step.\\
        \hline
    \end{tabular}
    \label{tab:notation}
\end{table}
